Co-Localization of Audio Sources in Images Using Binaural Features and Locally-Linear Regression

This paper addresses the problem of localizing audio sources using binaural measurements. We propose a supervised formulation that simultaneously localizes multiple sources at different locations. The approach is intrinsically efficient because, contrary to prior work, it relies neither on source separation, nor on monaural segregation. The method starts with a training stage that establishes a locally-linear Gaussian regression model between the directional coordinates of all the sources and the auditory features extracted from binaural measurements. While fixed-length wide-spectrum sounds (white noise) are used for training to reliably estimate the model parameters, we show that the testing (localization) can be extended to variable-length sparse-spectrum sounds (such as speech), thus enabling a wide range of realistic applications. Indeed, we demonstrate that the method can be used for audio-visual fusion, namely to map speech signals onto images and hence to spatially align the audio and visual modalities, thus enabling to discriminate between speaking and non-speaking faces. We release a novel corpus of real-room recordings that allow quantitative evaluation of the co-localization method in the presence of one or two sound sources. Experiments demonstrate increased accuracy and speed relative to several state-of-the-art methods.

==> mapping-antoineR2.tex <==
\subsection{Training With White-Noise Spectrograms}
\label{subsec:learn}
We now present the model that will be used to learn the relationship between binaural features and sound source directions using the acoustic space sampling dataset $\mathcal{T}_M$. This model belongs to the general family of \textit{Gaussian locally linear mapping} models introduced in [cite ArXiV]. The $(\yvect_n, \xvect_n)$ pairs in $\mathcal{T}_M$ are considered as realizations of random variables $(\Yvect,\Xvect)$. We define the following piecewise linear regression model from the low-dimensional multi-direction space to the high-dimensional $M-$acoustic space:
\begin{equation}
\label{eq:model_yxz}
  \Yvect=\sum_{k=1}^K \mathbb{I}(Z=k) (\Amat_k \Xvect + \bvect_k) + \Evect
\end{equation}
where matrix
$\Amat_k\in\mathbb{R}^{D\times L}$ and vector
$\bvect_k\in\mathbb{R}^D$ are the parameters of an affine transformation $\tau_k$ and
$\Evect\in\mathbb{R}^D$ is a Gaussian error vector with zero-mean and diagonal covariance
$\Sigmamat = \diag (\sigma^2_1 \hdots \sigma^2_d \hdots \sigma^2_D )$. $\Evect$
captures the
perturbations in $\mathbb{R}^D$ due to the variations of microphone noises and emitted sounds over time, as well as the reconstruction error
due to the local affine approximation. $\mathbb{I}$ is the indicator function and $Z$ is a hidden variable such that $\mathbb{I}(Z=k)=1$ if and only if $Z=k$ ($\Yvect$ is the transformed of $\Xvect$ by $\tau_k$), and $0$ otherwise. Consequently we have
\begin{equation}
\label{eq:learning_model_y}
p(\Yvect=\yvect|\Xvect=\xvect,Z=k) =
 \mathcal{N}(\yvect ;\Amat_k \xvect + \bvect_k ,\Sigmamat).
\end{equation}
To constrain the affine transformations to be local, we associate the $K$ affine transformations to an equal number of regions $\{\mathcal{R}_k\}_{k=1}^{k=K}\subset
\mathbb{R}^L$ that define a partitioning of $\mathcal{X}$. The regions are
modeled in a probabilistic way by assuming that $\Xvect$ follows
a mixture of $K$ Gaussians defined by
\begin{align}
\label{eq:priorXZsimple}
p(\Xvect=\xvect |Z=k) &= \mathcal{N}(\xvect ; \cvect_k,\Gammamat_k) \nonumber \\
p(Z=k) &= \pi_k
\end{align}
with $\cvect_k\in\mathbb{R}^L$, $\Gammamat_k\in\mathbb{R}^{L\times
L}$ and $\sum_k\pi_k=1$. In practice, $\pi_k$ is fixed to $1/K$ for all $k$, giving equal weights to all regions, but the remaining derivations are given in their generality.
This model yields an efficient EM algorithm referred to as \textit{probabilistic piecewise affine mapping} (PPAM) [CITE IJNS], which maximizes the observed-data log-likelihood $\log p(\{\yvect_n,\xvect_n\}_{n=1}^N ; \thetavect)$ with respect to the model's parameters:
\begin{equation}
 \label{eq:learning_model_Theta}
 \thetavect = \{\{\cvect_k,\Gammamat_k,\pi_k,\Amat_k,\bvect_k\}_{k=1}^K,\Sigmamat\}.
\end{equation}
At iteration $l+1$, the \textit{E-step} computes posterior probabilities $r_{kn}^{(l+1)} = p(z_{n}=k|\xvect_n,\yvect_n;\thetavect^{(l)})$, based on (\ref{eq:learning_model_y},\ref{eq:priorXZsimple}) and Bayes inversion. Then, the \textit{M-step} updates the parameters by $\thetavect^{(l+1)}=\operatorname*{argmax}_{\thetavect}[Q(\thetavect|\thetavect^{(l)})]$ where $Q(\thetavect|\thetavect^{(l)})$ denotes the expected complete-data log-likelihood given previous parameter estimates. Closed-form formulas for these steps are given in~[CITE IJNS].
%A locally affine partitioning obtained with PPAM on a toy dataset is shown in Fig.~\ref{fig:ppam}.
% \begin{figure}[t!]
% \centering
% \includegraphics[width = \linewidth,clip=,keepaspectratio]{figures/ppam.png}
% \caption{\label{fig:ppam}PPAM applied to a toy data set ($L=2,D=3,K=15$). Colors encode regions maximizing the final posterior probabilities $r_{kn}^{\infty}$ obtained after convergence of the algorithm. PPAM automatically adjusts these regions (associated with affine transformations) to the geometry of the data.}
% \end{figure}

\subsection{Forward Versus Inverse Mapping}
\label{subsec:inverse}
Given a set of parameters $\thetavect$, the mapping from a
multi-direction vector $\xvect\in\mathbb{R}^L$ to its corresponding mean binaural feature vector $\yvect\in\mathbb{R}^D$ is obtained using the
\textit{forward conditional density} of PPAM, \textit{i.e.}, $p(\yvect|\xvect;\thetavect)=$
\begin{equation}
 \label{eq:JGMM_forward_dens}
\sum_{k=1}^K \frac{\pi_k\mathcal{N}(\xvect ; \cvect_k,\Gammamat_k)}{\sum_{j=1}^K\pi_j\mathcal{N}(\xvect ; \cvect_j,\Gammamat_j)}\pi_k\mathcal{N}(\yvect;\Amat_k\xvect+\bvect_k,\Sigmamat).
\end{equation}
One can also map a mean binaural feature vector to its corresponding multi-direction vector using the \textit{inverse conditional density}, \textit{i.e.}, $p(\xvect|\yvect;\thetavect) =$
\begin{equation}
 \label{eq:JGMM_inverse_dens}
\sum_{k=1}^K \frac{\pi_k\mathcal{N}(\yvect ; \cvect_k^*,\Gammamat_k^*)}{\sum_{j=1}^K\pi_j\mathcal{N}(\yvect ; \cvect_j^*,\Gammamat^*_j)}\mathcal{N}(\xvect;\Amat^*_k\yvect+\bvect^*_k,\Sigmamat_k^*)
 \end{equation}
where $\cvect_k^{\ast}=\Amat_k\cvect_k+\bvect_k$,
$\Gammamat_k^{\ast}=\Sigmamat+\Amat_k\Gammamat_k\Amat_k\tp$,
$\Amat^{\ast}_k = \Sigmamat^{\ast}\Amat_k\tp\Sigmamat^{-1}$,
$\bvect^{\ast}_k =
\Sigmamat_k^*(\Gammamat_k^{-1}\cvect_k-\Amat_k\tp\Sigmamat^{-1}\bvect_k)$,
and $\Sigmamat_k^{\ast} =
(\Gammamat_k^{-1}+\Amat_k\tp\Sigmamat^{-1}\Amat_k)^{-1}$. Note
that both
(\ref{eq:JGMM_forward_dens}) and (\ref{eq:JGMM_inverse_dens}) take
the form of a Gaussian mixture distribution in one space given an observation in the other space.
These Gaussian mixtures are parameterized in two different ways by the
observed data and PPAM's parameters.
One can use their expectations to obtain
a \textit{forward mapping function} $\mathbb{E}[\Yvect=\yvect|\Xvect=\xvect;\thetavect]=$
\begin{equation}
 \label{eq:JGMM_forward_map}
 \sum_{k=1}^K \frac{\pi_k\mathcal{N}(\xvect ; \cvect_k,\Gammamat_k)}{\sum_{j=1}^K\pi_j\mathcal{N}(\xvect ; \cvect_j,\Gammamat_j)}(\Amat_k\xvect+\bvect_k),
\end{equation}
and more interestingly an \textit{inverse mapping function} $\mathbb{E}[\Xvect=\xvect|\Yvect=\yvect;\thetavect]=$
\begin{equation}
 \label{eq:JGMM_inverse_map}
 \sum_{k=1}^K \frac{\pi_k\mathcal{N}(\yvect ; \cvect_k^*,\Gammamat_k^*)}{\sum_{j=1}^K\pi_j\mathcal{N}(\yvect ; \cvect_j^*,\Gammamat^*_j)}(\Amat^*_k\yvect+\bvect^*_k).
\end{equation}
This possibility of learning the mapping from the low-dimensional space of multi-directions to the high-dimensional space of binaural features and then to inverse the mapping using (\ref{eq:JGMM_inverse_map}) is crucial. Indeed, let us consider a numerical example, where $K=10$, $L=2$ and $D=1000$. 
The number of parameters $\thetavect$ to estimate is then $K(1+L+DL+L(L+1)/2+D)=30,060$ using the proposed low-to-high dimensional mapping method. On the other hand, it would be $K(1+D+LD+D(D+1)/2+L)=5,035,030$ if the mapping was learned the other way around, requiring a huge amount of training data, and making the parameter estimation intractable.
\subsection{Mapping Binaural Spectrograms Onto Sound Directions}
\label{subsec:mapping}
PPAM combined with the inverse mapping formula (\ref{eq:JGMM_inverse_map}) allows to map a mean binaural feature vector $\yvect$ to its corresponding multi-direction vector $\xvect$. However, recall that this mean can only be obtained when $\chi_{dt}=1$ for all $(d,t)$, \textit{i.e.}, for wide-spectrum sound sources (see Section \ref{subsec:data}). We now address the more general problem of localizing mixtures of \textit{sparse-spectrum} sound sources, e.g., speech. We represent a recorded sound mixture by $\mathcal{S}=\{\ymat',\chimat\}$, where $\ymat'=\{y'_{dt}\}_{d=1,t=1}^{D,T}$ is the binaural feature spectrogram and $\chimat=\{\chi_{dt}\}_{d=1,t=1}^{D,T}$ denotes missing values. We seek the posterior density of the sound source directions,
$p(\xvect|\mathcal{S};\widetilde{\thetavect})$. We state and proof a theorem allowing for the full characterization of this density.
\begin{theorem}
\label{th:iPPAM}
Under the assumption that all the binaural features in 
$\mathcal{S}$ correspond to the same multi-direction vector, the posterior distribution 
%$p(\xvect|\mathcal{S};\widetilde{\thetavect})$ 
is a Gaussian mixture model in $\mathbb{R}^L$, namely
\begin{equation}
 \label{eq:spec_inv_GMM}
 p(\xvect|\mathcal{S};\widetilde{\thetavect})=\sum_{k=1}^K\nu_k\mathcal{N}(\xvect;\muvect_k,\Vmat_k).
\end{equation}
whose parameters $\{\nu_k, \muvect_k,\Vmat_k \}_{k=1}^{k=K}$ can be expressed in closed-form with respect to $\widetilde{\thetavect}$ and $\mathcal{S}$, namely:
\begin{eqnarray}
\label{eq:spectrogram_gmm_m}
\muvect_k &=& \Vmat_k\biggl(\widetilde{\Gammamat}_k^{-1}\widetilde{\cvect}_k+{\sum_{d,t=1}^{D,T}}\frac{\chi_{dt}}{\widetilde{\sigma}^2_{d}}\widetilde{\avect}_{dk}(y'_{dt}-\widetilde{b}_{dk})\biggr) \\
\label{eq:spectrogram_gmm_V}
\Vmat_k &=& \biggl(\widetilde{\Gammamat}_k^{-1}+{\sum_{d,t=1}^{D,T}}\frac{\chi_{dt}}{\widetilde{\sigma}^2_{d}}\widetilde{\avect}_{dk}\widetilde{\avect}_{dk}\tp\biggr)^{-1} \\
\label{eq:spectrogram_gmm_rho}
\nu_k & \propto  & \pi_k\frac{|\Vmat_k|^{\frac{1}{2}}}{|\widetilde{\Gammamat}_k|^{\frac{1}{2}}}\exp\biggl(-\frac{1}{2}\bigl(\sum_{d,t=1}^{D,T}\displaystyle\frac{\chi_{dt}}{\widetilde{\sigma}^2_{d}}(y'_{dt}-\widetilde{b}_{dk})^2 \nonumber \\
& +& \widetilde{\cvect}_k\tp\widetilde{\Gammamat}_k^{-1}\widetilde{\cvect}_k-\muvect_k\tp\Vmat_k^{-1}\muvect_k\bigr)\biggr)
\end{eqnarray}
where $\widetilde{\avect}\tp_{dk}\in\mathbb{R}^L$ is the $d^{th}$ row of $\widetilde{\Amat}_k$, $\tilde{b}_{dk}\in\mathbb{R}$ is the  $d^{th}$ entry of $\widetilde{\bvect}_k$ and $\nu_k$ is normalized so that $\sum_{k=1}^K\nu_k=1$.
\end{theorem}
A proof of Theorem~\ref{th:iPPAM} is given in Appendix \ref{app:th1}.

The posterior expectation can be used to estimate the sound sources image locations:
\begin{equation}
\label{eq:coloc}
 \widehat{\xvect}=\mathbb{E}[\xvect|\mathcal{S};\widetilde{\thetavect}]=\sum_{k=1}^K\nu_k\muvect_k.
\end{equation}
The corresponding technique will be referred to as \textit{visually supervised audio localization} or ViSuAL. ViSuAL-$M$ refer to the technique trained for $M$ simultaneous sound sources.

